Comprehensive language-image pre-training for 3D medical image understanding

In the 3D medical image domain, vision-language pre-training is used to create vision-language encoders (VLEs) that can support radiologists by retrieving patients with similar abnormalities, predicting likelihoods of abnormality, or, with downstream adaptation, generating radiological reports. While the methodology holds promise, three challenges limit the capabilities of current 3D VLEs: data scarcity due to privacy concerns, high computational costs resulting from the volumetric nature of the images, and a domain shift between the long reports used for training and the short prompts used during inference for, e.g., zero-shot classification. As a consequence, natural-image VLE recipes do not directly transfer to 3D medical imaging. In this paper, we overcome these challenges by injecting additional supervision via a report generation objective and combining vision-language with vision-only pre-training, allowing us to leverage both image-only and paired image-text 3D datasets. Further, we propose a novel loss that addresses the domain shift between long reports and short textual prompts. Through these additional objectives, paired with best practices of the 3D medical imaging domain, we develop the Comprehensive Language-Image Pre-training (COLIPRI) encoder family. Our COLIPRI encoders achieve state-of-the-art performance in report generation, semantic segmentation, classification probing, and zero-shot classification. The model weights and inference code are freely available at https://huggingface.co/microsoft/colipri.

==> figures/pca.tex <==

\newcommand{\pcafigwidth}{1}
\newlength{\figw}\setlength{\figw}{\pcafigwidth\textwidth}

\begin{figure*}[ht]
  \begin{minipage}{\figw}
  \centering
    \centering

    % --- config
    \newcommand{\pcawidth}{0.12} % column width fraction of \linewidth

    % --- helpers (paths include the pca/ folder)
    \newcommand{\imgct}[1]{figures/slices_pca_figure/ct_slice_#1.png}
    \newcommand{\imgmerlin}[1]{figures/slices_pca_figure/pca_merlin_ras_slice_#1.png}
    \newcommand{\imgctfm}[1]{figures/slices_pca_figure/pca_ct-fm_ras_slice_#1.png}
    \newcommand{\imgctclip}[1]{figures/slices_pca_figure/pca_ct-clip_ras_slice_#1.png}

    % \newcommand{\imgcolipriC}[1]{%
    %   figures/slices_pca_figure/pca_OptimizedClipTrainer_LLM_shuffle_p25__nnsslPlans__noresample_slice_#1.png}
    % \newcommand{\imgcolipriCM}[1]{%
    %   figures/slices_pca_figure/pca_OptimizedCLIPMAETrainer_160__nnsslPlans__noresample_slice_#1.png}
    % \newcommand{\imgcolipriCR}[1]{%
    %   figures/slices_pca_figure/pca_OptimizedCLIPCapTrainer_160__nnsslPlans__noresample_slice_#1.png}
    % \newcommand{\imgcolipriCRM}[1]{%
    %   figures/slices_pca_figure/pca_CLIPMAECAPTrainer_160__nnsslPlans__noresample_slice_#1.png}

    \newcommand{\imgcolipriC}[1]{%
      figures/slices_pca_figure/pca_OptimizedClipTrainerOpposedSentences__nnsslPlans__noresample_window_slice_#1.png}
    \newcommand{\imgcolipriCM}[1]{%
      figures/slices_pca_figure/pca_OptimizedCLIPMAETrainer_160_vo1_OS_random_MAEinit__nnsslPlans__noresample_window_slice_#1.png}
    \newcommand{\imgcolipriCR}[1]{%
      figures/slices_pca_figure/pca_OptimizedCLIPCapTrainer_160_OS__nnsslPlans__noresample_window_slice_#1.png}
    \newcommand{\imgcolipriCRM}[1]{%
      figures/slices_pca_figure/pca_CLIPMAECAPTrainer_160_OS_vo1_MAEinit__nnsslPlans__noresample_window_slice_#1.png}

    % reference heights from a non-Merlin column (match Merlin height)
    \newlength{\colw}\setlength{\colw}{\pcawidth\linewidth}
    \newsavebox{\refsag}
    \sbox{\refsag}{\includegraphics[width=\colw]{\imgctclip{sagittal}}}
    \newlength{\Hsag}\setlength{\Hsag}{\ht\refsag}
    \newsavebox{\refcor}
    \sbox{\refcor}{\includegraphics[width=\colw]{\imgctclip{coronal}}}
    \newlength{\Hcor}\setlength{\Hcor}{\ht\refcor}

    % ---------- Row 1: sagittal (no subcaptions)
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgct{sagittal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth,height=\Hsag]{\imgmerlin{sagittal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgctfm{sagittal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \usebox{\refsag}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriC{sagittal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriCR{sagittal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriCM{sagittal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriCRM{sagittal}}
    \end{subfigure}

    \vspace{0.6ex}

    % ---------- Row 2: coronal (no subcaptions)
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgct{coronal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth,height=\Hcor]{\imgmerlin{coronal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgctfm{coronal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \usebox{\refcor}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriC{coronal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriCR{coronal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriCM{coronal}}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriCRM{coronal}}
    \end{subfigure}

    \vspace{0.6ex}

    % Make captions a bit smaller
    \captionsetup[subfigure]{font=scriptsize, justification=centering, singlelinecheck=false}

    % ---------- Row 3: axial (with subcaptions + labels)
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgct{axial}}
      \caption{Input}\label{fig:pca:input}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgmerlin{axial}}
      \caption{Merlin}\label{fig:pca:merlin}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgctfm{axial}}
      \caption{CT-FM}\label{fig:pca:ctfm}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgctclip{axial}}
      \caption{CT-CLIP}\label{fig:pca:ctclip}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriC{axial}}
      \caption{COLIPRI-C}\label{fig:pca:colipri-c}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriCR{axial}}
      \caption{COLIPRI-CR}\label{fig:pca:colipri-cr}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriCM{axial}}
      \caption{COLIPRI-CM}\label{fig:pca:colipri-cm}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{\pcawidth\linewidth}
      \centering
      \includegraphics[width=\linewidth]{\imgcolipriCRM{axial}}
      \caption{COLIPRI-CRM}\label{fig:pca:colipri-crm}
    \end{subfigure}

  \caption{
    \textbf{
        \Ac{PCA} maps of dense 3D features
    }
    obtained from a CT scan with a lung mass \subref{fig:pca:input} using different encoders.
    Compared to the baseline methods \subref{fig:pca:merlin}\subref{fig:pca:ctfm}\subref{fig:pca:ctclip}, the \method models \subref{fig:pca:colipri-c} \subref{fig:pca:colipri-cm} \subref{fig:pca:colipri-cr} \subref{fig:pca:colipri-crm} generate sharper and more coherent features.
    The dense embeddings have sizes 7$\times$7$\times$10 \subref{fig:pca:merlin}, 24$\times$24$\times$8 \subref{fig:pca:ctfm}, 24$\times$24$\times$24 \subref{fig:pca:ctclip} and 48$\times$48$\times$48 \subref{fig:pca:colipri-c}, \subref{fig:pca:colipri-cm}, \subref{fig:pca:colipri-cr}, \subref{fig:pca:colipri-crm} and are interpolated here using bicubic interpolation for visualisation purposes.
  }
  \label{fig:pca}
  \end{minipage}
\end{figure*}

==> tables/all_results_tables.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{l|ccc|cc|cc|cc}
    \toprule
    Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
    Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\\midrule
    Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
    no LPE & 9.27 & 23.48 & 33.33 & 55.38 & 83.20 & 43.30 & 76.18 & 25.07 & 58.56 \\
    \bottomrule
    \end{tabular}

    \caption{Stage 1: Learnable positional embeddings}
    \label{tab:placeholder}
\end{table*}


\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
CXR-BERT from scratch & \multicolumn{9}{c}{Did not converge }\\
BiomedCLIP & 3.43 & 13.28 & 19.47 & 52.79 & 81.89 & 37.43 & 74.21 & 28.16 & 59.30 \\
\bottomrule
\end{tabular}


    \caption{Stage 1: Other text encoders}
    \label{tab:placeholder}
\end{table*}




\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
Short sentence p10& 9.94 & 25.90 & 34.25 & 55.70 & 83.50 & 47.97 & 78.98 & 37.29 & 69.51 \\
Short sentence p25 & 7.60 & 25.15 & 35.25 & 57.07 & 83.96 & 49.54 & 80.21 & 41.18 & 74.65 \\
Short sentence p50 & 5.93 & 22.89 & 33.42 & 57.60 & 84.23 & 50.97 & 80.90 & 39.84 & 71.02 \\
Short sentence p75 & 4.51 & 15.20 & 25.23 & 57.31 & 84.02 & 51.70 & 80.91 & 36.04 & 65.21 \\
\bottomrule
\end{tabular}

    \caption{Short sentence augmentation }
    \label{tab:placeholder}
\end{table*}

\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
Short sent. LLM & 2.59 & 9.28 & 16.05 & 50.78 & 80.94 & 44.33 & 78.06 & 33.16 & 67.84 \\
Short sent. LLM p25 & 2.84 & 11.29 & 17.64 & 51.11 & 81.25 & 44.72 & 76.95 & 33.98 & 64.68 \\
Short sent. LLM p25 neg & 2.01 & 9.62 & 18.48 & 52.32 & 81.94 & 43.67 & 78.05 & 41.59 & 72.91 \\
Short sent. LLM p50 & 4.01 & 15.72 & 24.25 & 55.03 & 83.01 & 47.49 & 78.82 & 31.78 & 62.58 \\
Short sent. LLM p75 & 4.93 & 16.89 & 25.59 & 54.81 & 83.14 & 47.58 & 78.27 & 31.42 & 66.68 \\
\bottomrule
\end{tabular}


    \caption{Short sentence augmentation through an LLM. *neg indicates using short sentences denoted as negative as well.}
    \label{tab:placeholder}
\end{table*}

\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
trainer &  &  &  &  &  &  &  &  &  \\
\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
AveragePooling & 5.93 & 18.88 & 27.90 & 54.34 & 83.03 & 40.20 & 75.48 & 35.65 & 67.46 \\
MaxPooling & 11.45 & 27.57 & 38.01 & 56.18 & 83.56 & 42.80 & 75.32 & 25.86 & 56.57 \\
Learned AP & 5.68 & 16.12 & 25.15 & 53.77 & 82.97 & 40.51 & 75.78 & 30.60 & 61.87 \\
Learned AP + MaxPool & 6.77 & 22.14 & 30.49 & 54.47 & 83.09 & 41.98 & 76.22 & 31.95 & 62.29 \\
MaxPool AP & 5.18 & 19.88 & 28.24 & 54.72 & 83.13 & 44.31 & 77.09 & 32.05 & 62.16 \\
4Token Learned AP& 5.60 & 16.96 & 24.64 & 53.64 & 82.87 & 40.34 & 75.05 & 33.28 & 62.90 \\
SingleHead AP & 5.43 & 19.13 & 27.57 & 54.05 & 82.82 & 40.84 & 75.83 & 33.27 & 62.19 \\

\bottomrule
\end{tabular}

\caption{Stage 1: Various forms of pooling of dense tokens for Language Alignment.}
    \label{tab:placeholder}
\end{table*}

\begin{table*}
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
2x Steps& 8.52 & 21.97 & 28.57 & 55.94 & 83.63 & 41.52 & 74.57 & 27.68 & 59.39 \\
16x16x16 Patches& 5.76 & 14.62 & 22.14 & 49.88 & 81.05 & 40.71 & 75.12 & 29.58 & 61.80 \\
2x Learning Rate & 3.09 & 12.45 & 21.55 & 53.28 & 82.29 & 41.81 & 76.10 & 23.34 & 51.38 \\
2x LR + high WD & 5.01 & 14.20 & 22.39 & 53.72 & 82.69 & 43.62 & 76.73 & 21.69 & 48.62 \\

\bottomrule

\end{tabular}
\caption{Stage 1: Auxiliary Hparams.}
    \label{tab:placeholder}
\end{table*}


\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule
Default & 7.94 & 23.64 & 32.75 & 55.91 & 83.51 & 43.22 & 76.24 & 34.77 & 66.70 \\
Label Smoothing .005 & 9.02 & 25.23 & 33.92 & 56.24 & 83.51 & 36.74 & 70.62 & 26.49 & 59.48 \\
Label Smoothing .01 & 9.61 & 24.64 & 33.17 & 56.28 & 83.55 & 39.16 & 72.04 & 25.59 & 58.85 \\
Label Smoothing .02 & 7.94 & 22.89 & 33.00 & 55.61 & 83.43 & 40.30 & 73.10 & 27.13 & 56.55 \\
\bottomrule
\end{tabular}


    \caption{Stage 1: Label smoothing}
    \label{tab:placeholder}
\end{table*}

\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
Input Size 160 & 7.94 & 23.64 & 32.75 & 55.91 & 83.51 & 43.22 & 76.24 & 34.77 & 66.70 \\
Input Size 128 & 8.35 & 22.06 & 29.66 & 56.19 & 83.78 & 44.60 & 77.17 & 32.00 & 63.05 \\
\bottomrule
\end{tabular}

    \caption{Stage 1: Input Size}
    \label{tab:placeholder}
\end{table*}

\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
trainer &  &  &  &  &  &  &  &  &  \\
\midrule
(low) DA Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
normal DA & 9.02 & 22.47 & 30.49 & 55.73 & 83.65 & 43.43 & 76.05 & 31.90 & 63.28 \\
high DA & 4.59 & 15.96 & 23.73 & 54.91 & 83.11 & 41.44 & 76.16 & 30.71 & 59.63 \\

\bottomrule
\end{tabular}

    \caption{Effect of Data augmentation.}
    \label{tab:placeholder}
\end{table*}

\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
BS16 2xlr .5 steps & 9.77 & 24.98 & 32.75 & 55.66 & 83.44 & 41.68 & 75.48 & 31.82 & 63.40 \\
BS24 3xlr .33 steps& 8.10 & 23.89 & 31.75 & 55.95 & 83.51 & 43.13 & 76.05 & 30.87 & 62.27 \\
BS32 4xlr .25 steps & 8.27 & 20.05 & 29.32 & 55.19 & 83.23 & 40.55 & 74.77 & 23.69 & 53.89 \\
BS128 \@ 128 LR 2.4e-4 & 8.44 & 20.13 & 26.57 & DnF & DnF & DnF & DnF & DnF & DnF \\
\bottomrule
\end{tabular}
    \caption{Effect of Batch size scaling.}
    \label{tab:placeholder}
\end{table*}

\begin{table*}[]
    \centering
    \begin{tabular}{l|ccc|cc|cc|cc}
    \toprule
    Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
    Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
    \midrule
    Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
    SigLIP & 5.60 & 16.21 & 24.06 & 53.88 & 82.81 & 39.45 & 74.66 & 30.90 & 63.44 \\
    \bottomrule
    \end{tabular}

    \caption{CLIP vs SigLIP loss.}
    \label{tab:placeholder}
\end{table*}

\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R1 & R5 & R10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
Short Sentence + shuffle + neg & 12.71 & 29.01 & 39.30 & 56.91 & 83.76 & 45.81 & 77.93 & 39.55 & 71.15 \\
Short Sentence + shuffle + neg p25 & 11.54 & 27.68 & 38.04 & 56.45 & 83.87 & 47.12 & 78.67 & 35.13 & 68.10 \\
Short Sentence + shuffle + neg p50 & 11.20 & 28.01 & 38.21 & 56.32 & 83.91 & 46.07 & 78.63 & 37.09 & 70.24 \\
Short Sentence + shuffle + neg p75 & 9.78 & 25.92 & 34.36 & 56.97 & 84.01 & 46.41 & 78.74 & 34.70 & 68.19 \\
\bottomrule
\end{tabular}




    \caption{LLM sentence shorten with negatives and shuffling}
    \label{tab:placeholder}
\end{table*}


\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R@1 & R@5 & R@10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
Optimized CLIP & 11.03 & 25.90 & 34.67 & 58.02 & 84.23 & 46.55 & 78.33 & 38.29 & 71.95 \\

\bottomrule
\end{tabular}




    \caption{CLIP Optimization results compared to the initial default configuration. Optimized CLIP refers to our \textit{'OptimizedClipTrainer LLM shuffle p10'} trainer. }
    \label{tab:placeholder}
\end{table*}


\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R@1 & R@5 & R@10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
Optimized CLIP & 11.03 & 25.90 & 34.67 & 58.02 & 84.23 & 46.55 & 78.33 & 38.29 & 71.95 \\
Optimized CLIP + CapPa & 16.12 & 32.50 & 42.44 & 56.58 & 83.70 & 44.59 & 76.43 & 33.11 & 70.46 \\


\bottomrule
\end{tabular}

    \caption{CLIP Optimization results compared to the initial default configuration. Optimized CLIP refers to our \textit{'OptimizedClipTrainer LLM shuffle p10'} trainer.}
    \label{tab:placeholder}
\end{table*}


\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R@1 & R@5 & R@10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
our CLIP & 11.03 & 25.90 & 34.67 & 58.02 & 84.23 & 46.55 & 78.33 & 38.29 & 71.95 \\
our CLIP + CapPa & 16.12 & 32.50 & 42.44 &  56.58 & 83.70 & 44.59 & 76.43 & 33.11 & 70.46 \\
our CLIP + MAE & 14.79 & 30.66 & 39.01 &56.29 & 83.52 & 40.94 & 74.86 & 37.03 & 72.66 \\



\bottomrule
\end{tabular}

    \caption{CLIP Optimization results compared to the initial default configuration. Optimized CLIP refers to our \textit{'OptimizedClipTrainer LLM shuffle p10'} trainer.}
    \label{tab:placeholder}
\end{table*}


\begin{table*}[]
    \centering
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
Eval & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-shot (A)} & \multicolumn{2}{r}{Zero-shot (S)} \\
Metric & R@1 & R@5 & R@10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule
Default & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\
our CLIP & 11.03 & 25.90 & 34.67 & 58.02 & 84.23 & 46.55 & 78.33 & 38.29 & 71.95 \\
our CLIP + CapPa & 16.12 & 32.50 & 42.44 &  56.58 & 83.70 & 44.59 & 76.43 & 33.11 & 70.46 \\
our CLIP + MAE & 14.79 & 30.66 & 39.01 &56.29 & 83.52 & 40.94 & 74.86 & 37.03 & 72.66 \\
\bottomrule
\end{tabular}

    \caption{Generation Performance}
    \label{tab:placeholder}
\end{table*}



\begin{table*}[]
    \centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{l|cccccc}
\toprule
Metric & IJEPA & Merlin & old CLIP & CLIP & Clip+MAE & CLIP+CapPa \\
\midrule
Micro$F_1$ & 27.1 [25.9, 28.3] & 28.0 [26.7, 29.4] & 33.6 [32.4, 35.2] & 34.0 [32.7, 35.5] & 29.9 [28.7, 31.3] & 34.5 [33.4, 35.9] \\
ROUGE-L & 31.0 [30.3, 31.6] & 31.1 [30.5, 31.7] & 31.7 [31.0, 32.3] & 31.7 [30.9, 32.6] & 30.9 [30.3, 31.7] & 31.8 [30.9, 32.5] \\
\bottomrule
\end{tabular}
}

    \caption{Generation results with latest clip models. Generation results with Qwen 2.5 - 1.5B backbone with Perceiver style token aggregation. }
    \label{tab:placeholder}
\end{table*}


==> tables/classification_test_results.tex <==
\begin{tabular}{l|cc|cc}
\toprule
Model & \multicolumn{2}{c|}{\ctrate} & \multicolumn{2}{c}{\radchestct} \\
 & AUROC & Bal. ACC & AUROC & Bal. ACC \\
\midrule
Baseline (S) & 60.30 & 58.10 & 54.10 & 53.90 \\
CT-VocabFine (S) & 75.00 & 69.20 & 64.90 & 62.20 \\
CT-LiPro (S) & 75.10 & 67.60 & 64.70 & 62.50 \\
CT-CLIP (Z) & 70.40 & 65.10 & 63.20 & 59.90 \\
BIUD (Z) & 71.30 & 68.10 & 62.90 & 60.60 \\
Merlin (Z) & 72.80 & 67.20 & 64.40 & 61.90 \\
fVLM (Z) & 77.80 & 71.80 & 68.00 & 64.70 \\\midrule
Clip Sim. (Z) & 71.30 & 65.00 & 66.67 & 60.64 \\
Clip Adv. (Z) & 77.51 & 70.02 & 67.15 & 61.47 \\
Clip (S) & 83.88 & 74.75 & 72.80 & 65.14 \\\midrule
Clip+MAE Sim. (Z) & 72.02 & 66.43 & 64.60 & 60.11 \\
Clip+MAE Adv. (Z) & 74.87 & 68.64 & 65.97 & 60.57 \\
Clip+MAE (S) & 83.38 & 74.43 & 72.11 & 64.67 \\\midrule
Clip+Cap Sim. (Z) & 69.77 & 65.09 & 60.08 & 57.28 \\
Clip+Cap Adv. (Z) & 75.27 & 68.54 & 66.93 & 60.99 \\
Clip+Cap (S) & 83.67 & 74.13 & 72.16 & 64.77 \\
\bottomrule
\end{tabular}


==> tables/clipcap/clipcap_depth.tex <==
\begin{tabular}{lrrrllllll}
\toprule
setting & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-Shot Simple} & \multicolumn{2}{r}{Zero-Shot Advanced} \\
Generator Depth & R@1 & R@5 & R@10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
\midrule

 4 & NaN & NaN & NaN & 55.85 & 83.40 & 37.69 & 69.41 & 46.29 & 76.53 \\
 6 & NaN & NaN & NaN & 55.72 & 83.28 & 34.56 & 69.39 & 44.73 & 75.88 \\
 8 & NaN & NaN & NaN & 54.14 & 82.59 & 31.23 & 60.90 & 45.20 & 75.80 \\
 12 & NaN & NaN & NaN & 55.09 & 82.89 & 32.94 & 66.49 & 43.87 & 75.35 \\
\bottomrule
\end{tabular}


==> tables/clipcap/clipcap_step_ratio.tex <==
\begin{tabular}{lrrrllllll}
\toprule
setting & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-Shot Simple} & \multicolumn{2}{r}{Zero-Shot Advanced} \\
Cap-CapPa Ratio  & R@1 & R@5 & R@10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\ 
\midrule

0-100 & NaN & NaN & NaN & 54.53 & 82.80 & 35.11 & 63.22 & 44.66 & 74.97 \\
25-75 & NaN & NaN & NaN & 54.27 & 73.52 & 29.28 & 61.28 & 43.48 & 75.59 \\
50-50 & NaN & NaN & NaN & 55.09 & 82.89 & 32.94 & 66.49 & 43.87 & 75.35 \\
75-25 & NaN & NaN & NaN & 55.32 & 83.28 & 35.82 & 68.63 & 45.80 & 77.03 \\
100-0 & NaN & NaN & NaN & 56.36 & 83.42 & 31.13 & 61.41 & 44.89 & 75.64 \\
\bottomrule
\end{tabular}


==> tables/clipcap/clipcap_weight.tex <==
\begin{tabular}{lrrrllllll}
\toprule
setting & \multicolumn{3}{r}{Retrieval} & \multicolumn{2}{r}{Lin. Probe} & \multicolumn{2}{r}{Zero-Shot Simple} & \multicolumn{2}{r}{Zero-Shot Advanced} \\
$\lambda_{\text{RRG}}$ & R@1 & R@5 & R@10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\
Trainer &  &  &  &  &  &  &  &  &  \\
\midrule
Loss weight 0.1 & NaN & NaN & NaN & 55.79 & 83.14 & 33.65 & 64.59 & 45.56 & 76.43 \\
Loss weight 0.3 & NaN & NaN & NaN & 55.29 & 83.17 & 36.46 & 68.09 & 45.38 & 76.70 \\
Loss weight 1 & NaN & NaN & NaN & 55.09 & 82.89 & 32.94 & 66.49 & 43.87 & 75.35 \\
\bottomrule
\end{tabular}


==> tables/maxs_cis_files/cls_probes_ctrate_with_CIs.tex <==
\begin{tabular}{lccccc}
\toprule
metric & AUPRC & AUROC & $F_1$ & Pr & Rc \\
trainer &  &  &  &  &  \\
\midrule
OptimizedClipTrainer LLM shuffle p10 & 57.37 [55.84, 58.82] & 83.88 [83.11, 84.37] & 57.95 [57.44, 59.81] & 52.38 [51.13, 56.03] & 67.87 [64.72, 70.67] \\
OptimizedCLIPCapTrainer 160 & 56.98 [55.61, 58.91] & 83.67 [83.07, 84.30] & 57.53 [56.98, 59.49] & 53.94 [51.29, 56.43] & 64.49 [63.05, 69.39] \\
OptimizedCLIPMAETrainer 160 & 56.37 [54.88, 58.11] & 83.38 [82.72, 84.18] & 56.84 [56.36, 58.82] & 51.40 [49.64, 54.29] & 65.51 [64.42, 70.17] \\
\bottomrule
\end{tabular}


==> tables/maxs_cis_files/cls_probes_radchestct_with_CIs.tex <==
\begin{tabular}{lccccc}
\toprule
metric & AUPRC & AUROC & $F_1$ & Pr & Rc \\
trainer &  &  &  &  &  \\
\midrule
OptimizedClipTrainer LLM shuffle p10 & 48.57 [47.97, 49.45] & 72.80 [72.19, 73.34] & 51.37 [51.14, 52.45] & 44.40 [43.83, 46.50] & 70.12 [67.35, 72.40] \\
OptimizedCLIPCapTrainer 160 & 47.49 [46.69, 48.30] & 72.16 [71.69, 72.68] & 50.42 [50.04, 51.47] & 42.86 [42.17, 44.60] & 69.76 [67.14, 72.63] \\
OptimizedCLIPMAETrainer 160 & 47.35 [46.44, 48.35] & 72.11 [71.50, 72.60] & 50.02 [49.71, 51.07] & 42.22 [41.29, 43.96] & 69.09 [66.35, 72.42] \\
\bottomrule
\end{tabular}


==> tables/optimizing_clip_table.tex <==
\begin{table*}
\centering
\caption{\textbf{Optimizing CLIP.} Due to the domain gap between natural imaging and 3D medical imaging, we reinvestigate key aspects of the CLIP method, yielding an optimized CLIP variant. In this table we only highlight the most relevant changes, for all ablations we defer to \TODO{Add ref to appendix.}}
\label{tab:optimizing_clip}

\resizebox{\linewidth}{!}{\begin{tabular}{l|ccc|cc|cc|cc}
     & \multicolumn{3}{c}{Retrieval} & \multicolumn{2}{c}{Lin. Cls. Probe} & \multicolumn{2}{c}{Zero-shot Cls. (N)} & \multicolumn{2}{c}{Zero-shot Cls. (S)} \\
 Change & R@1 & R@5 & R@10 & AUPRC & AUROC & AUPRC & AUROC & AUPRC & AUROC \\\midrule
    \rowcolor{gray!30}Default  & 8.27 & 22.64 & 31.66 & 55.41 & 83.11 & 43.48 & 76.48 & 34.77 & 66.91 \\\midrule
    BS 16; x2 LR; /2 Steps & 9.77 & 24.98 & 32.75 & 55.66 & 83.44 & 41.68 & 75.48 & 31.82 & 63.40 \\
    + Sentence Shuffle & 11.11 & 28.57 & 37.93 & 56.66 & 83.94 & 44.05 & 76.55 & 35.13 & 69.21 \\
    + Sentence Shuffle + Sentence Shorten & 12.71 & 29.01 & 39.30 & 56.91 & 83.76 & 45.81 & 77.93 & 39.55 & 71.15 \\
    More image data aug. & 9.02 & 22.47 & 30.49 & 55.73 & 83.65 & 43.43 & 76.05 & 31.90 & 63.28 \\
    - no absolute Positional Embedding & 9.27 & 23.48 & 33.33 & 55.38 & 83.20 & 43.30 & 76.18 & 25.07 & 58.56 \\\midrule
    \textbf{Optimized CLIP} & 11.03 & 25.90 & 34.67 & 58.02 & 84.23 & 46.55 & 78.33 & 38.29 & 71.95 \\
\end{tabular}}



\end{table*}


==> tables/preliminary_retrieval.tex <==


\begin{table*}[]
    \centering
\resizebox{.7\linewidth}{!}{\begin{tabular}{lcccccccc}
\toprule

trainer & AUPRC & AUROC & $F_1$ & Pr & Rc & BA & BAA & $F_1$ (CTCLIP) \\
\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP BS16 lrx2 epdiv2 & \underline{55.66} & 83.44 & 57.15 & 49.87 & 68.94 & 75.39 & 50.77 & 79.16 \\
CLIP BS24 lrx3 epdiv3 & \textbf{55.95} & 83.51 & 57.64 & 50.19 & 69.57 & 75.51 & 51.02 & 79.17 \\
CLIP BS32 lrx4 epdiv4 & 55.19 & 83.23 & 56.56 & 51.50 & 65.16 & 73.74 & 47.48 & 78.75 \\\midrule
\rowcolor{gray!20}CLIP  & \underline{55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP AvgPool  & 54.34 & 83.03 & 56.62 & 50.50 & 68.16 & 74.62 & 49.24 & 78.37 \\
CLIP MaxPool  & \textbf{56.18} & 83.56 & 57.48 & 52.13 & 67.52 & 74.30 & 48.61 & 79.01 \\
CLIP LQA  & 53.77 & 82.97 & 56.08 & 49.99 & 66.17 & 73.91 & 47.82 & 78.66 \\
CLIP LQAMaxPool1D  & 54.47 & 83.09 & 56.35 & 50.25 & 66.27 & 73.95 & 47.91 & 78.59 \\
CLIP MaxPoolQueryAP  & 54.72 & 83.13 & 56.58 & 50.74 & 66.80 & 74.45 & 48.91 & 78.73 \\
CLIP MultiLQA  & 53.64 & 82.87 & 56.16 & 49.22 & 68.24 & 74.55 & 49.09 & 78.55 \\
CLIP SingleHeadAP1D  & 54.05 & 82.82 & 56.17 & 49.55 & 68.75 & 74.60 & 49.21 & 78.78 \\\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP defaultDA &\textbf{55.73} & 83.65 & 57.10 & 49.99 & 69.27 & 75.51 & 51.02 & 79.92 \\
CLIP BS8 DA5 & 54.91 & 83.11 & 56.51 & 50.20 & 67.39 & 74.47 & 48.94 & 79.17 \\\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
+ sentence shuffling & \textbf{56.66} & 83.94 & 57.92 & 52.38 & 67.24 & 74.76 & 49.52 & \underline{79.45} \\
+ Sam's cleaned & 55.24 & 83.00 & 56.77 & 50.34 & 66.72 & 74.18 & 48.36 & 78.88 \\
+ Sam's cleaned shuffled & \underline{56.21} & 83.64 & 57.05 & 52.13 & 65.65 & 74.20 & 48.41 & 79.15 \\
+ short sentence & 56.03 & 83.57 & 57.54 & 51.05 & 69.42 & 74.99 & 49.99 & 78.81 \\
+ short sentence shuffle & 55.70 & 83.50 & 57.21 & 51.29 & 66.37 & 74.80 & 49.59 & \textbf{79.48} \\
+ ibrahim structured report & 55.65 & 82.97 & 56.45 & 50.56 & 66.86 & 74.19 & 48.38 & 78.03 \\
+ ibrahim structured report shuffled & 55.87 & 83.30 & 56.91 & 50.30 & 67.04 & 74.52 & 49.04 & 79.10 \\\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP  2000ep & \textbf{55.94} & 83.63 & 57.17 & 50.11 & 69.80 & 75.10 & 50.19 & 78.85 \\\midrule
\rowcolor{gray!20}CLIP  & \textbf{55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP  imp. & 54.89 & 83.29 & 56.94 & 50.71 & 68.09 & 74.91 & 49.83 & 79.65 \\
CLIP  find. imp. & \underline{55.31} & 83.27 & 57.16 & 49.32 & 70.56 & 75.34 & 50.69 & 79.04 \\\midrule
\rowcolor{gray!20}CLIP  & \textbf{55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP BioMedCLIP  & 52.79 & 81.89 & 54.86 & 47.47 & 68.15 & 73.60 & 47.20 & 77.79 \\\midrule
\rowcolor{gray!20}CLIP  &\textbf{55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
Clip  lr6e5 & 53.28 & 82.29 & 55.37 & 48.67 & 68.91 & 73.68 & 47.36 & 77.91 \\
Clip  lr6e5 wd5e2 & 53.72 & 82.69 & 55.93 & 49.96 & 67.70 & 74.27 & 48.54 & 78.57 \\\midrule
\rowcolor{gray!20}CLIP  & \textbf{55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
Clip frozen T & 54.68 & 82.98 & 56.21 & 50.85 & 65.04 & 73.59 & 47.19 & 78.32 \\\midrule
\rowcolor{gray!20}CLIP  &\textbf{ 55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
SigLIP  & 53.88 & 82.81 & 56.41 & 50.65 & 66.16 & 74.30 & 48.61 & 78.70 \\\midrule
CLIP BS8 128 & \textbf{56.19} & 83.78 & 57.35 & 50.10 & 70.12 & 75.48 & 50.96 & 79.42 \\
CLIP BS8 160 & \underline{55.91} & 83.51 & 57.05 & 50.00 & 69.38 & 74.62 & 49.25 & 78.99 \\
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP BS8 224 & 54.44 & 83.06 & 56.93 & 51.64 & 66.08 & 74.40 & 48.79 & 78.50 \\\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP Patchsize 16 & 49.88 & 81.05 & 53.84 & 46.48 & 66.93 & 72.92 & 45.84 & 77.51 \\\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
+ noLPE & 55.38 & 83.20 & 56.68 & 50.46 & 68.52 & 74.13 & 48.26 & 78.39 \\\midrule
CLIP 160 & 55.91 & 83.51 & 57.05 & 50.00 & 69.38 & 74.62 & 49.25 & 78.99 \\
+ label smooth .005 & 56.24 & 83.51 & 56.88 & 51.42 & 67.02 & 74.53 & 49.06 & 78.90 \\
+ label smooth .01 & \textbf{56.28} & 83.55 & 57.18 & 51.76 & 67.67 & 74.60 & 49.21 & 78.80 \\
+ label smooth .02 & 55.61 & 83.43 & 57.31 & 50.60 & 68.61 & 75.14 & 50.28 & 79.40 \\\midrule
\rowcolor{red!20}Final & \textbf{57.72} &\textbf{ 84.20} & \textbf{58.45} & \textbf{52.81} & 68.08 & 75.18 & 50.37 & 79.47 \\


\bottomrule
\end{tabular}}



    \caption{Classification results when training a linear classification }
    \label{tab:linear_classification_probe_clip}
\end{table*}



\begin{table*}[]
    \centering
\resizebox{.7\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule

trainer & AUPRC & AUROC & $F_1$ & Pr & Rc & BA & BAA & $F_1$ (CTCLIP) \\
\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP BS16 lrx2 epdiv2 & \underline{55.66} & 83.44 & 57.15 & 49.87 & 68.94 & 75.39 & 50.77 & 79.16 \\
CLIP BS24 lrx3 epdiv3 & \textbf{55.95} & 83.51 & 57.64 & 50.19 & 69.57 & 75.51 & 51.02 & 79.17 \\
CLIP BS32 lrx4 epdiv4 & 55.19 & 83.23 & 56.56 & 51.50 & 65.16 & 73.74 & 47.48 & 78.75 \\\midrule
\rowcolor{gray!20}CLIP  & \underline{55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP AvgPool  & 54.34 & 83.03 & 56.62 & 50.50 & 68.16 & 74.62 & 49.24 & 78.37 \\
CLIP MaxPool  & \textbf{56.18} & 83.56 & 57.48 & 52.13 & 67.52 & 74.30 & 48.61 & 79.01 \\
CLIP LQA  & 53.77 & 82.97 & 56.08 & 49.99 & 66.17 & 73.91 & 47.82 & 78.66 \\
CLIP LQAMaxPool1D  & 54.47 & 83.09 & 56.35 & 50.25 & 66.27 & 73.95 & 47.91 & 78.59 \\
CLIP MaxPoolQueryAP  & 54.72 & 83.13 & 56.58 & 50.74 & 66.80 & 74.45 & 48.91 & 78.73 \\
CLIP MultiLQA  & 53.64 & 82.87 & 56.16 & 49.22 & 68.24 & 74.55 & 49.09 & 78.55 \\
CLIP SingleHeadAP1D  & 54.05 & 82.82 & 56.17 & 49.55 & 68.75 & 74.60 & 49.21 & 78.78 \\\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP defaultDA &\textbf{55.73} & 83.65 & 57.10 & 49.99 & 69.27 & 75.51 & 51.02 & 79.92 \\
CLIP BS8 DA5 & 54.91 & 83.11 & 56.51 & 50.20 & 67.39 & 74.47 & 48.94 & 79.17 \\\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
+ sentence shuffling & \textbf{56.66} & 83.94 & 57.92 & 52.38 & 67.24 & 74.76 & 49.52 & \underline{79.45} \\
+ Sam's cleaned & 55.24 & 83.00 & 56.77 & 50.34 & 66.72 & 74.18 & 48.36 & 78.88 \\
+ Sam's cleaned shuffled & \underline{56.21} & 83.64 & 57.05 & 52.13 & 65.65 & 74.20 & 48.41 & 79.15 \\
+ short sentence & 56.03 & 83.57 & 57.54 & 51.05 & 69.42 & 74.99 & 49.99 & 78.81 \\
+ short sentence shuffle & 55.70 & 83.50 & 57.21 & 51.29 & 66.37 & 74.80 & 49.59 & \textbf{79.48} \\
+ ibrahim structured report & 55.65 & 82.97 & 56.45 & 50.56 & 66.86 & 74.19 & 48.38 & 78.03 \\
+ ibrahim structured report shuffled & 55.87 & 83.30 & 56.91 & 50.30 & 67.04 & 74.52 & 49.04 & 79.10 \\\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP  2000ep & \textbf{55.94} & 83.63 & 57.17 & 50.11 & 69.80 & 75.10 & 50.19 & 78.85 \\\midrule
\rowcolor{gray!20}CLIP  & \textbf{55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP  imp. & 54.89 & 83.29 & 56.94 & 50.71 & 68.09 & 74.91 & 49.83 & 79.65 \\
CLIP  find. imp. & \underline{55.31} & 83.27 & 57.16 & 49.32 & 70.56 & 75.34 & 50.69 & 79.04 \\\midrule
\rowcolor{gray!20}CLIP  & \textbf{55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP BioMedCLIP  & 52.79 & 81.89 & 54.86 & 47.47 & 68.15 & 73.60 & 47.20 & 77.79 \\\midrule
\rowcolor{gray!20}CLIP  &\textbf{55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
Clip  lr6e5 & 53.28 & 82.29 & 55.37 & 48.67 & 68.91 & 73.68 & 47.36 & 77.91 \\
Clip  lr6e5 wd5e2 & 53.72 & 82.69 & 55.93 & 49.96 & 67.70 & 74.27 & 48.54 & 78.57 \\\midrule
\rowcolor{gray!20}CLIP  & \textbf{55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
Clip frozen T & 54.68 & 82.98 & 56.21 & 50.85 & 65.04 & 73.59 & 47.19 & 78.32 \\\midrule
\rowcolor{gray!20}CLIP  &\textbf{ 55.41} & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
SigLIP  & 53.88 & 82.81 & 56.41 & 50.65 & 66.16 & 74.30 & 48.61 & 78.70 \\\midrule
CLIP BS8 128 & \textbf{56.19} & 83.78 & 57.35 & 50.10 & 70.12 & 75.48 & 50.96 & 79.42 \\
CLIP BS8 160 & \underline{55.91} & 83.51 & 57.05 & 50.00 & 69.38 & 74.62 & 49.25 & 78.99 \\
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP BS8 224 & 54.44 & 83.06 & 56.93 & 51.64 & 66.08 & 74.40 & 48.79 & 78.50 \\\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
CLIP Patchsize 16 & 49.88 & 81.05 & 53.84 & 46.48 & 66.93 & 72.92 & 45.84 & 77.51 \\\midrule
\rowcolor{gray!20}CLIP  & 55.41 & 83.11 & 56.86 & 49.36 & 70.15 & 74.81 & 49.62 & 78.59 \\
+ noLPE & 55.38 & 83.20 & 56.68 & 50.46 & 68.52 & 74.13 & 48.26 & 78.39 \\\midrule
CLIP 160 & 55.91 & 83.51 & 57.05 & 50.00 & 69.38 & 74.62 & 49.25 & 78.99 \\
+ label smooth .005 & 56.24 & 83.51 & 56.88 & 51.42 & 67.02 & 74.53 & 49.06 & 78.90 \\
+ label smooth .01 & \textbf{56.28} & 83.55 & 57.18 & 51.76 & 67.67 & 74.60 & 49.21 & 78.80 \\
+ label smooth .02 & 55.61 & 83.43 & 57.31 & 50.60 & 68.61 & 75.14 & 50.28 & 79.40 \\\midrule
\rowcolor{red!20}Final & \textbf{57.72} &\textbf{ 84.20} & \textbf{58.45} & \textbf{52.81} & 68.08 & 75.18 & 50.37 & 79.47 \\


\bottomrule
\end{tabular}}



    \caption{Classification results when training a linear classification }
    \label{tab:linear_classification_probe_clip}
\end{table*}


\begin{table*}[]
    \centering
\resizebox{.7\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
metric & \multicolumn{2}{c|}{AUPRC} & \multicolumn{2}{c|}{AUROC} & \multicolumn{2}{c|}{$F_1$} & \multicolumn{2}{c|}{bal. acc. adj.} \\
prompt style & adv & simple & adv & simple & adv & simple & adv & simple \\
trainer &  &  &  &  &  &  &  &  \\
\midrule\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP BS16 lrx2 epdiv2 & 41.68 & 31.82 & 75.48 & 63.40 & 48.60 & 38.86 & 38.09 & 21.54 \\
CLIP BS24 lrx3 epdiv3 & 43.13 & 30.87 & 76.05 & 62.27 & 49.37 & 37.53 & 39.41 & 19.67 \\
CLIP BS32 lrx4 epdiv4 & 40.55 & 23.69 & 74.77 & 53.89 & 47.53 & 32.81 & 37.10 & 8.27 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP AveragePool BS8 & 40.20 & 35.65 & 75.48 & 67.46 & 46.90 & 40.27 & 38.42 & 26.06 \\
CLIP MaxPool BS8 & 42.80 & 25.86 & 75.32 & 56.57 & 48.33 & 35.76 & 37.59 & 13.17 \\
CLIP LQA BS8 & 40.51 & 30.60 & 75.78 & 61.87 & 48.42 & 37.02 & 39.52 & 19.84 \\
CLIP LQAMaxPool1D BS8 & 41.98 & 31.95 & 76.22 & 62.29 & 49.39 & 36.77 & 39.40 & 17.26 \\
CLIP MaxPoolQA BS8 & 44.31 & 32.05 & 77.09 & 62.16 & 50.56 & 37.10 & 39.94 & 18.89 \\
CLIP MultiLQA BS8 & 40.34 & 33.28 & 75.05 & 62.90 & 47.18 & 37.78 & 38.02 & 20.86 \\
CLIP 1HeadAP BS8 & 40.84 & 33.27 & 75.83 & 62.19 & 48.74 & 38.10 & 39.33 & 22.24 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP BS8 defaultDA & 43.43 & 31.90 & 76.05 & 63.28 & 49.50 & 38.69 & 39.12 & 21.86 \\
CLIP BS8 DA5 & 41.44 & 30.71 & 76.16 & 59.63 & 48.64 & 38.62 & 39.43 & 19.76 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP BS8 sentence shuffling & 44.05 & 35.13 & 76.55 & 69.21 & 49.84 & 41.51 & 38.69 & 28.25 \\
CLIP BS8 cleaned & 42.69 & 28.29 & 76.29 & 60.11 & 49.04 & 36.94 & 38.18 & 16.83 \\
CLIP BS8 cleaned shuffled & 44.22 & 32.05 & 76.73 & 67.19 & 49.73 & 39.40 & 39.14 & 26.23 \\
CLIP BS8 findings impressions & 43.64 & 31.39 & 76.74 & 67.64 & 49.71 & 40.83 & 40.69 & 27.68 \\
CLIP BS8 impressions & 43.74 & 29.11 & 76.52 & 62.40 & 50.37 & 36.72 & 39.60 & 19.91 \\
CLIP BS8 short sentence & 47.61 & 37.46 & 78.54 & 70.51 & 52.88 & 43.96 & 43.46 & 32.25 \\
CLIP BS8 short sentence shuffle & 47.97 & 37.29 & 78.98 & 69.51 & 52.73 & 43.67 & 45.08 & 30.68 \\
CLIP BS8 short sentence shuffle p25 & 49.54 & 41.18 & 80.21 & 74.65 & 54.33 & 47.61 & 46.15 & 36.15 \\
CLIP BS8 short sentence shuffle p50 & 50.97 & 39.84 & 80.90 & 71.02 & 55.28 & 45.61 & 46.85 & 34.59 \\
CLIP BS8 short sentence shuffle p75 & 51.70 & 36.04 & 80.91 & 65.21 & 55.04 & 42.87 & 47.37 & 27.15 \\
CLIP BS8 short sentence llm & 44.33 & 33.16 & 78.06 & 67.84 & 50.37 & 41.93 & 42.47 & 29.38 \\
CLIP BS8 short sentence llm p25 & 44.72 & 33.98 & 76.95 & 64.68 & 49.96 & 41.88 & 41.34 & 26.88 \\
CLIP BS8 short sentence llm p50 & 47.49 & 31.78 & 78.82 & 62.58 & 51.85 & 41.06 & 41.66 & 21.96 \\
CLIP BS8 short sentence llm p75 & 47.58 & 31.42 & 78.27 & 66.68 & 51.64 & 40.54 & 41.77 & 26.16 \\
CLIP BS8 short sentence llm p25 neg & 43.67 & 41.59 & 78.05 & 72.91 & 50.05 & 47.75 & 41.96 & 34.95 \\
ibrahim structured & 43.68 & 28.93 & 76.81 & 62.91 & 49.91 & 37.81 & 40.75 & 21.07 \\
ibrahim structured shuffled & 44.43 & 34.55 & 77.69 & 68.89 & 50.50 & 40.75 & 41.51 & 27.70 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP BS8 2000ep & 41.52 & 27.68 & 74.57 & 59.39 & 48.07 & 35.05 & 35.39 & 14.48 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP BioMedCLIP BS8 & 37.43 & 28.16 & 74.21 & 59.30 & 45.87 & 35.35 & 37.57 & 15.13 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP BS8 lr6e5 & 41.81 & 23.34 & 76.10 & 51.38 & 49.01 & 33.88 & 40.67 & 9.56 \\
CLIP BS8 lr6e5 wd5e2 & 43.62 & 21.69 & 76.73 & 48.62 & 49.93 & 32.28 & 40.10 & 5.82 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP BS8 frozen softmax temp & 43.09 & 31.90 & 76.60 & 64.04 & 49.62 & 39.30 & 39.08 & 23.04 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
SigLip BS8 & 39.45 & 30.90 & 74.66 & 63.44 & 47.69 & 39.17 & 38.80 & 19.78 \\\midrule
CLIP BS8 128 & 44.60 & 32.00 & 77.17 & 63.05 & 50.35 & 37.63 & 40.64 & 20.11 \\
CLIP BS8 160 & 43.22 & 34.77 & 76.24 & 66.70 & 50.07 & 40.69 & 40.74 & 26.04 \\
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP BS8 224 & 42.69 & 29.99 & 76.13 & 64.78 & 49.58 & 38.10 & 40.06 & 23.52 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP BS8 PS16 & 40.71 & 29.58 & 75.12 & 61.80 & 47.81 & 37.23 & 36.15 & 18.20 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP noLPE BS8 & 43.30 & 25.07 & 76.18 & 58.56 & 49.33 & 34.89 & 38.66 & 14.55 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 34.77 & 76.48 & 66.91 & 50.29 & 40.95 & 41.19 & 26.09 \\
CLIP BS8 160 label smooth 005 & 36.74 & 26.49 & 70.62 & 59.48 & 42.72 & 35.13 & 29.36 & 14.61 \\
CLIP BS8 160 label smooth 01 & 39.16 & 25.59 & 72.04 & 58.85 & 44.79 & 35.81 & 31.28 & 15.45 \\
CLIP BS8 160 label smooth 02 & 40.30 & 27.13 & 73.10 & 56.55 & 46.07 & 34.61 & 32.99 & 12.89 \\\midrule
\rowcolor{red!30}Final CLIP & \textbf{48.34} & 36.98 & 79.18 & 68.28 & 52.82 & 42.96 & 44.03 & 28.45 \\
\bottomrule
\end{tabular}
}



    \caption{Zero-shot classification results on the validation set of the CT-Rate dataset. Metrics represent the average across abnormalities.}
    \label{tab:my_label}
\end{table*}

\begin{table*}[]
    \centering
    \resizebox{.7\linewidth}{!}{
    \begin{tabular}{l|cccccccc}
\toprule
metric & AUPRC & AUROC & $F_1$ & Pr & Rc & bal. acc. & bal. acc. adj. & $F_1$ (CTCLIP) \\
\midrule\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP BS16 lrx2 epdiv2 & 31.82 & 63.40 & 38.86 & 29.82 & 68.82 & 60.77 & 21.54 & 65.44 \\
CLIP BS24 lrx3 epdiv3 & 30.87 & 62.27 & 37.53 & 27.17 & 77.49 & 59.84 & 19.67 & 65.90 \\
CLIP BS32 lrx4 epdiv4 & 23.69 & 53.89 & 32.81 & 23.21 & 76.13 & 54.13 & 8.27 & 60.69 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP AveragePool BS8 & 35.65 & 67.46 & 40.27 & 30.80 & 63.58 & 63.03 & 26.06 & 68.03 \\
CLIP MaxPool BS8 & 25.86 & 56.57 & 35.76 & 27.60 & 70.39 & 56.58 & 13.17 & 61.45 \\
CLIP LQA BS8 & 30.60 & 61.87 & 37.02 & 26.93 & 72.44 & 59.92 & 19.84 & 64.03 \\
CLIP LQAMaxPool1D BS8 & 31.95 & 62.29 & 36.77 & 26.54 & 73.87 & 58.63 & 17.26 & 65.74 \\
CLIP MaxPoolQueryAttention BS8 & 32.05 & 62.16 & 37.10 & 29.27 & 64.82 & 59.45 & 18.89 & 65.57 \\
CLIP MultiLQA BS8 & 33.28 & 62.90 & 37.78 & 29.38 & 62.24 & 60.43 & 20.86 & 67.42 \\
CLIP 1HeadAP BS8 & 33.27 & 62.19 & 38.10 & 28.48 & 66.55 & 61.12 & 22.24 & 65.94 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP BS8 defaultDA & 31.90 & 63.28 & 38.69 & 30.00 & 66.32 & 60.93 & 21.86 & 66.14 \\
CLIP BS8 DA5 & 30.71 & 59.63 & 38.62 & 28.50 & 73.38 & 59.88 & 19.76 & 62.50 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP BS8 sentence shuffling & 35.13 & 69.21 & 41.51 & 31.86 & 67.05 & 64.13 & 28.25 & 69.25 \\
CLIP BS8 cleaned & 28.29 & 60.11 & 36.94 & 27.86 & 70.49 & 58.42 & 16.83 & 63.00 \\
CLIP BS8 cleaned shuffled & 32.05 & 67.19 & 39.40 & 28.78 & 69.09 & 63.12 & 26.23 & 67.39 \\
CLIP BS8 findings impressions & 31.39 & 67.64 & 40.83 & 30.19 & 65.62 & 63.84 & 27.68 & 68.15 \\
CLIP BS8 impressions & 29.11 & 62.40 & 36.72 & 25.47 & 74.90 & 59.95 & 19.91 & 64.94 \\
CLIP BS8 short sentence & 37.46 & 70.51 & 43.96 & 33.92 & 75.62 & 66.12 & 32.25 & 69.35 \\
CLIP BS8 short sentence shuffle & 37.29 & 69.51 & 43.67 & 35.19 & 71.27 & 65.34 & 30.68 & 69.43 \\
CLIP BS8 short sentence shuffle p25 & 41.18 & 74.65 & 47.61 & 38.88 & 66.40 & 68.07 & 36.15 & 73.27 \\
CLIP BS8 short sentence shuffle p50 & 39.84 & 71.02 & 45.61 & 37.99 & 65.01 & 67.30 & 34.59 & 71.76 \\
CLIP BS8 short sentence shuffle p75 & 36.04 & 65.21 & 42.87 & 33.76 & 74.12 & 63.58 & 27.15 & 68.57 \\
CLIP BS8 short sentence llm & 33.16 & 67.84 & 41.93 & 32.33 & 64.96 & 64.69 & 29.38 & 68.88 \\
CLIP BS8 short sentence llm p25 & 33.98 & 64.68 & 41.88 & 33.22 & 66.34 & 63.44 & 26.88 & 67.83 \\
CLIP BS8 short sentence llm p50 & 31.78 & 62.58 & 41.06 & 32.26 & 75.02 & 60.98 & 21.96 & 67.76 \\
CLIP BS8 short sentence llm p75 & 31.42 & 66.68 & 40.54 & 30.31 & 72.00 & 63.08 & 26.16 & 66.91 \\
CLIP BS8 short sentence llm p25 neg & 41.59 & 72.91 & 47.75 & 40.43 & 68.09 & 67.48 & 34.95 & 73.91 \\
ibrahim structured shuffled & 34.55 & 68.89 & 40.75 & 29.99 & 66.84 & 63.85 & 27.70 & 67.24 \\
ibrahim structured & 28.93 & 62.91 & 37.81 & 27.82 & 67.40 & 60.54 & 21.07 & 65.29 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP BS8 2000ep & 27.68 & 59.39 & 35.05 & 25.58 & 74.96 & 57.24 & 14.48 & 62.78 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP BioMedCLIP BS8 & 28.16 & 59.30 & 35.35 & 26.00 & 70.67 & 57.57 & 15.13 & 64.09 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP BS8 lr6e5 & 23.34 & 51.38 & 33.88 & 23.34 & 79.21 & 54.78 & 9.56 & 59.80 \\
CLIP BS8 lr6e5 wd5e2 & 21.69 & 48.62 & 32.28 & 21.08 & 83.04 & 52.91 & 5.82 & 56.22 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP BS8 frozen softmax temp & 31.90 & 64.04 & 39.30 & 29.78 & 69.53 & 61.52 & 23.04 & 65.74 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
SigLip BS8 & 30.90 & 63.44 & 39.17 & 30.61 & 65.07 & 59.89 & 19.78 & 66.28 \\\midrule
CLIP BS8 128 & 32.00 & 63.05 & 37.63 & 29.58 & 63.61 & 60.06 & 20.11 & 66.17 \\
CLIP BS8 160 & 34.77 & 66.70 & 40.69 & 31.42 & 67.72 & 63.02 & 26.04 & 67.13 \\
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP BS8 224 & 29.99 & 64.78 & 38.10 & 27.01 & 71.27 & 61.76 & 23.52 & 66.53 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP BS8 PS16 & 29.58 & 61.80 & 37.23 & 26.94 & 66.53 & 59.10 & 18.20 & 65.03 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP noLPE BS8 & 25.07 & 58.56 & 34.89 & 24.49 & 71.60 & 57.27 & 14.55 & 62.71 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 34.77 & 66.91 & 40.95 & 32.36 & 66.44 & 63.04 & 26.09 & 68.50 \\
CLIP BS8 160 label smooth 005 & 26.49 & 59.48 & 35.13 & 25.52 & 67.23 & 57.31 & 14.61 & 63.89 \\
CLIP BS8 160 label smooth 01 & 25.59 & 58.85 & 35.81 & 25.78 & 76.54 & 57.73 & 15.45 & 62.82 \\
CLIP BS8 160 label smooth 02 & 27.13 & 56.55 & 34.61 & 25.89 & 64.90 & 56.44 & 12.89 & 62.82 \\\midrule
Final CLIP & 36.98 & 68.28 & 42.96 & 33.89 & 71.75 & 64.22 & 28.45 & 68.33 \\

\bottomrule
\end{tabular}}
    \caption{Zero-shot classification with simple prompt only. Prompt: "\{Abnormality\} is present" vs "No \{Abnormality\} is present.".}
    \label{tab:my_label}
\end{table*}

\begin{table*}[]
    \centering
    \resizebox{.7\linewidth}{!}{
    \begin{tabular}{lcccccccc}
\toprule
metric & AUPRC & AUROC & $F_1$ & Pr & Rc & bal. acc. & bal. acc. adj. & $F_1$ (CTCLIP) \\
\midrule\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP BS16 lrx2 epdiv2 & 41.68 & 75.48 & 48.60 & 40.07 & 65.56 & 69.04 & 38.09 & 73.85 \\
CLIP BS24 lrx3 epdiv3 & 43.13 & 76.05 & 49.37 & 40.89 & 65.81 & 69.70 & 39.41 & 74.51 \\
CLIP BS32 lrx4 epdiv4 & 40.55 & 74.77 & 47.53 & 39.36 & 66.57 & 68.55 & 37.10 & 73.06 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP AveragePool BS8 & 40.20 & 75.48 & 46.90 & 36.57 & 68.25 & 69.21 & 38.42 & 72.82 \\
CLIP MaxPool BS8 & 42.80 & 75.32 & 48.33 & 40.40 & 65.28 & 68.80 & 37.59 & 72.60 \\
CLIP LQA BS8 & 40.51 & 75.78 & 48.42 & 39.30 & 68.30 & 69.76 & 39.52 & 73.86 \\
CLIP LQAMaxPool1D BS8 & 41.98 & 76.22 & 49.39 & 41.07 & 65.20 & 69.70 & 39.40 & 74.61 \\
CLIP MaxPoolQueryAttention BS8 & 44.31 & 77.09 & 50.56 & 42.15 & 66.38 & 69.97 & 39.94 & 74.44 \\
CLIP MultiLQA BS8 & 40.34 & 75.05 & 47.18 & 38.34 & 67.07 & 69.01 & 38.02 & 73.60 \\
CLIP 1HeadAP BS8 & 40.84 & 75.83 & 48.74 & 39.39 & 67.93 & 69.66 & 39.33 & 74.19 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP BS8 defaultDA & 43.43 & 76.05 & 49.50 & 41.27 & 67.97 & 69.56 & 39.12 & 74.19 \\
CLIP BS8 DA5 & 41.44 & 76.16 & 48.64 & 39.35 & 67.17 & 69.72 & 39.43 & 74.39 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP BS8 sentence shuffling & 44.05 & 76.55 & 49.84 & 42.38 & 65.70 & 69.34 & 38.69 & 73.93 \\
CLIP BS8 cleaned & 42.69 & 76.29 & 49.04 & 41.55 & 63.51 & 69.09 & 38.18 & 73.91 \\
CLIP BS8 cleaned shuffled & 44.22 & 76.73 & 49.73 & 41.49 & 66.72 & 69.57 & 39.14 & 74.45 \\
CLIP BS8 findings impressions & 43.64 & 76.74 & 49.71 & 40.02 & 69.76 & 70.35 & 40.69 & 74.70 \\
CLIP BS8 impressions & 43.74 & 76.52 & 50.37 & 42.84 & 66.08 & 69.80 & 39.60 & 74.48 \\
CLIP BS8 short sentence & 47.61 & 78.54 & 52.88 & 44.78 & 68.31 & 71.73 & 43.46 & 76.34 \\
CLIP BS8 short sentence shuffle & 47.97 & 78.98 & 52.73 & 44.06 & 69.95 & 72.54 & 45.08 & 76.28 \\
CLIP BS8 short sentence shuffle p25 & 49.54 & 80.21 & 54.33 & 46.63 & 67.62 & 73.07 & 46.15 & 77.31 \\
CLIP BS8 short sentence shuffle p50 & 50.97 & 80.90 & 55.28 & 48.15 & 67.55 & 73.43 & 46.85 & 78.28 \\
CLIP BS8 short sentence shuffle p75 & 51.70 & 80.91 & 55.04 & 47.61 & 67.51 & 73.69 & 47.37 & 77.36 \\
CLIP BS8 short sentence llm & 44.33 & 78.06 & 50.37 & 40.59 & 70.31 & 71.24 & 42.47 & 74.91 \\
CLIP BS8 short sentence llm p25 & 44.72 & 76.95 & 49.96 & 40.80 & 69.58 & 70.67 & 41.34 & 74.94 \\
CLIP BS8 short sentence llm p50 & 47.49 & 78.82 & 51.85 & 45.31 & 65.56 & 70.83 & 41.66 & 75.30 \\
CLIP BS8 short sentence llm p75 & 47.58 & 78.27 & 51.64 & 44.51 & 66.72 & 70.88 & 41.77 & 75.52 \\
CLIP BS8 short sentence llm p25 neg & 43.67 & 78.05 & 50.05 & 41.49 & 67.72 & 70.98 & 41.96 & 74.62 \\
ibrahim structured shuffled & 44.43 & 77.69 & 50.50 & 41.98 & 66.69 & 70.75 & 41.51 & 75.13 \\
ibrahim structured & 43.68 & 76.81 & 49.91 & 40.29 & 70.02 & 70.38 & 40.75 & 74.14 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP BS8 2000ep & 41.52 & 74.57 & 48.07 & 40.38 & 65.47 & 67.69 & 35.39 & 73.36 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP BioMedCLIP BS8 & 37.43 & 74.21 & 45.87 & 34.94 & 70.57 & 68.79 & 37.57 & 72.32 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP BS8 lr6e5 & 41.81 & 76.10 & 49.01 & 39.39 & 69.03 & 70.34 & 40.67 & 74.31 \\
CLIP BS8 lr6e5 wd5e2 & 43.62 & 76.73 & 49.93 & 41.28 & 67.87 & 70.05 & 40.10 & 74.31 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP BS8 frozen softmax temp & 43.09 & 76.60 & 49.62 & 41.66 & 65.38 & 69.54 & 39.08 & 73.55 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
SigLip BS8 & 39.45 & 74.66 & 47.69 & 38.44 & 67.46 & 69.40 & 38.80 & 73.84 \\\midrule
CLIP BS8 128 & 44.60 & 77.17 & 50.35 & 41.89 & 66.98 & 70.32 & 40.64 & 75.18 \\
CLIP BS8 160 & 43.22 & 76.24 & 50.07 & 41.14 & 68.53 & 70.37 & 40.74 & 74.48 \\
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP BS8 224 & 42.69 & 76.13 & 49.58 & 40.60 & 67.69 & 70.03 & 40.06 & 74.76 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP BS8 PS16 & 40.71 & 75.12 & 47.81 & 39.36 & 65.18 & 68.08 & 36.15 & 72.90 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP noLPE BS8 & 43.30 & 76.18 & 49.33 & 40.64 & 67.58 & 69.33 & 38.66 & 74.26 \\\midrule
\rowcolor{gray!30} CLIP BS8 & 43.48 & 76.48 & 50.29 & 40.95 & 69.90 & 70.59 & 41.19 & 74.52 \\
CLIP BS8 160 label smooth 005 & 36.74 & 70.62 & 42.72 & 33.73 & 62.79 & 64.68 & 29.36 & 70.14 \\
CLIP BS8 160 label smooth 01 & 39.16 & 72.04 & 44.79 & 37.63 & 61.77 & 65.64 & 31.28 & 70.17 \\
CLIP BS8 160 label smooth 02 & 40.30 & 73.10 & 46.07 & 39.04 & 60.41 & 66.50 & 32.99 & 71.82 \\\midrule
Final CLIP & \textbf{48.34} & \textbf{79.18} & \underline{52.82} & 44.56 & 67.58 & 72.02 & 44.03 & 76.13 \\
\bottomrule
\end{tabular}
    }
    \caption{Zero-shot classification performance with the "Advanced" prompts. These are 30 randomly chosen reports that are positive for the abnormality of interest and 30 randomly chosen reports that are negative for the abnormality of interest. For each of these other abnormalities may or may not be present.}
    \label{tab:my_label}
\end{table*}


==> tables/results/classification_old.tex <==
\begin{tabular}{l|llll|llll}
\toprule
 & \multicolumn{4}{c|}{CT-RATE} & \multicolumn{4}{c}{RAD-ChestCT} \\
 & AUPRC & AUROC & BA & $F_1$ & AUPRC & AUROC & BA & $F_1$ \\
\midrule
MedImageInsights & 19.70 & 50.52 & 52.00 & 31.25 & 27.94 & 52.25 & 52.26 & 39.17 \\
Curia & 45.93 & 78.01 & 69.91 & 50.29 & 39.23 & 65.73 & 59.98 & 45.36 \\
CT-CLIP & 25.96 & 61.21 & 57.66 & 34.49 & 28.77 & 54.05  & 52.65 & 39.08 \\
CT-CLIP (reported) & - & 75.1 & 67.6 & - & - & 64.7 & 62.5 & - \\
CT-FM & 53.54 & 82.14 & 73.51 & 55.56 & 42.41 & 68.49 & 61.95 & 47.55 \\
Merlin & 54.81 & 82.62 & 74.28 & 56.69 & 45.30 & 70.91 & 64.34 & 49.35 \\\midrule
\cellcolor{microsoftred!20}{\colipric} & 57.41 & 84.15 & 74.99 & \textbf{57.99} & \textbf{48.86} & \textbf{72.66} & \textbf{65.17} & \textbf{51.31} \\
\cellcolor{microsoftblue!20}{\colipricr} & \underline{56.98} & \underline{83.67} & 74.13 & \underline{57.53} & 47.49 & 72.16 & 64.77 & 50.42 \\
\cellcolor{microsoftgreen!20}{\colipricm} & 56.37 & 83.38 & 74.43 & 56.84 & 47.35 & 72.11 & 64.67 & 50.02 \\
\cellcolor{microsoftyellow!20}{\colipricrm} & 56.65 & 83.31 & \underline{74.88} & 57.31 & \underline{47.99} & \underline{72.40} & \underline{64.86} & \underline{50.99} \\
\bottomrule
\end{tabular}


==> tables/results/segmentation_short.tex <==
\begin{tabular}{l|rrrr}
\toprule
Trainer & \textbf{LiTS} & \textbf{Lung} & \textbf{HVS} & \textbf{KiTS23} \\
\midrule
\multicolumn{3}{l}{\textbf{References} (250k steps)} \\
nnU-Net Default & 80.09 & 70.32 & 68.38 & 86.04 \\
nnU-Net ResEnc-L & 81.60 & 70.34 & 67.73 & 88.17 \\
\midrule
\multicolumn{2}{l}{\textbf{Primus-M} (37.5k steps)} \\
From scratch & 74.39 & 62.74 & 64.67 & 78.90 \\
%Primus-M scratch 1k & 79.75 & 69.11 & 65.34 & 86.25 \\
MAE & \underline{80.27} & 67.12 & \textbf{67.10} & 85.34 \\
\cellcolor{microsoftred!20}{\colipric} & 76.77 & 65.89 & 64.64 & 81.02 \\
\cellcolor{microsoftblue!20}{\colipricr} & 77.09 & 65.32 & 65.08 & 80.71 \\
\cellcolor{microsoftgreen!20}{\colipricm} & 79.97 & \underline{68.74} & 66.58 & \textbf{86.03} \\
\rowcolor{gray!15}\cellcolor{microsoftyellow!20}{\colipricrm }  & \textbf{80.46} & \textbf{68.98} & \underline{67.05} & \underline{85.79} \\\midrule
\multicolumn{2}{l}{\textbf{Primus-M} (250k steps)} \\
From scratch & 79.75 & \textbf{69.11} & 65.34 & 86.25 \\
MAE & \underline{80.32} & 67.46 & \underline{65.73} & \underline{87.46} \\
\rowcolor{gray!15}\cellcolor{microsoftyellow!20}{\colipricrm } & \textbf{81.11} & \underline{67.56} & \textbf{66.42} & \textbf{87.68} \\
\bottomrule
\end{tabular}


==> tables/results/test_retrieval.tex <==
\begin{tabular}{lrrr}
\toprule
 & R@1 & R@5 & R@10 \\
\midrule

CT-CLIP & - & 2.90 & 5.00 \\
\cellcolor{microsoftred!20}\colipric & 4.49 & 13.46 & 19.69 \\
\cellcolor{microsoftblue!20}\colipricr & 7.23 & 19.36 & 26.99 \\
\cellcolor{microsoftgreen!20}\colipricm & 14.53 & 34.16 & 45.34 \\
\rowcolor{gray!15}\cellcolor{microsoftyellow!20}\colipricrm & \textbf{15.27} & \textbf{35.10} & \textbf{46.01} \\

\bottomrule
\end{tabular}


==> tables/results/zeroshot_classification_main_old.tex <==
\begin{tabular}{ll|ccc|ccc}
\toprule
yes & & \multicolumn{3}{c|}{CT-RATE} & \multicolumn{3}{c}{RAD-ChestCT} \\
 Model & PS & AUROC & BA & w-$F_1$ & AUROC & BA & w-$F_1$ \\
\midrule
MedImageInsights & short & 49.36 & 51.49 & 31.08 & 48.82 & 50.24 & 38.34 \\ 
MedImageInsights & native & 49.99 & 51.09 & 31.02 & 49.93 & 50.33 & 38.36 \\
Curia & short & 50.17 & 51.25 & 31.03
 & 50.13 & 50.67 & 38.45 \\ 
Curia & native & 50.27 & 51.24 & 31.03 & 50.29 & 50.63 & 38.40 \\
CT-CLIP & - & 70.4$^*$ & 65.1$^*$ &  69.1$^*$ & 63.2$^*$ & 59.9$^*$ &  64.8$^*$ \\
BIUD & - & 71.3$^*$ & 68.1$^*$ & 71.6$^*$ & 62.9$^*$ & 60.6$^*$ & 65.2$^*$ \\
Merlin & - & 72.8$^*$ & 67.2$^*$ &  70.9$^*$ & 64.4$^*$ & \underline{61.9}$^*$ & 66.3$^*$ \\
fVLM & - & \textbf{77.8}$^*$ & \textbf{71.8}$^*$ & 75.1$^*$ & \textbf{68.0}$^*$ & \textbf{64.7}$^*$ & \textbf{68.8}$^*$ \\\midrule
\cellcolor{microsoftred!20}{\colipric} & short & 70.18 & 64.87 & 69.13 & 63.09 & 58.56 & 63.85 \\
\cellcolor{microsoftred!20}{\colipric} & native & \textbf{77.80} & \underline{70.15}& \textbf{75.20} & \underline{66.98} & 60.94 & 65.73 \\
\cellcolor{microsoftblue!20}{\colipricr} & short & 69.77 & 65.09 & 67.91 & 60.08 & 57.28 & 61.53 \\
\cellcolor{microsoftblue!20}{\colipricr} & native & \underline{75.27} & 68.54 & 74.22 & 66.93 & 60.99 & \underline{66.48} \\
\cellcolor{microsoftgreen!20}{\colipricm} & short & 72.02 & 66.43 & 70.58 & 64.60 & 60.11 & 65.03 \\
\cellcolor{microsoftgreen!20}{\colipricm} & native & 74.87 & 68.64 & 73.62 & 65.97 & 60.56 & 65.93 \\
\cellcolor{microsoftyellow!20}{\colipricrm } & short & 71.86 & 66.54 & 70.92 & 63.22 & 58.91 & 64.70 \\
\cellcolor{microsoftyellow!20}{\colipricrm} & native & 75.02 & 68.50 & 74.39 & 66.47 & 60.51 & 66.05 \\
\bottomrule
\end{tabular}


==> tables/short_ablations.tex <==


% 1. We ablate SigLIPv2 vs CLIP
% 2. Ablate BatchSize
% 3. Ablate TokenPooling
% 4. Impressions, Find+Impressions
% 5. noLPE vs LPE
% 6. Text Augmentation

